Tangent Convolutions for Dense Prediction in 3D

We present an approach to semantic scene analysis using deep convolutional networks. Our approach is based on tangent convolutions - a new construction for convolutional networks on 3D data. In contrast to volumetric approaches, our method operates directly on surface geometry. Crucially, the construction is applicable to unstructured point clouds and other noisy real-world data. We show that tangent convolutions can be evaluated efficiently on large-scale point clouds with millions of points. Using tangent convolutions, we design a deep fully-convolutional network for semantic segmentation of 3D point clouds, and apply it to challenging real-world datasets of indoor and outdoor 3D environments. Experimental results show that the presented approach outperforms other recent deep network constructions in detailed analysis of large 3D scenes.

==> tex/implementation.tex <==
%So far, we have introduced the essential mathematical operations of our framework: convolution and pooling.
%In this section we define the standard neural network layers based on these operations.
Conventional 2D CNNs operate on feature maps of size $W \times H \times C$\footnote{Here we omit the mini-batch dimension for simplicity}, where $W, H$ are the spatial dimensions and $C$ is the number of channels.
Instead, our networks operate on $N \times C$ arrays where $N$ is the number of points in the point cloud.
A neural network layer transforms an input feature map $F_{in}$ of size $N_{in} \times C_{in}$ into an output feature map $F_{out}$ of size $N_{out} \times C_{out}$.

Equation~\ref{eq:convolution} amount to defining a regular structure in tangent plane and estimating signal values at elements of this domain based on the signal values of corresponding points.
This observation allows us to formulate a unified way of implementing CNN layers.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/implementation.jpg}
\caption{Implementation.}
\label{fig:implementation}
\end{figure}

Consider a local operation $O$ with a kernel comprised of K elements.
It can be a $k \times k$ kernel of a 2D convolution, or a $k \times k \times k$ kernel of the pooling operation.
To apply this operation to a point cloud, we assemble an $N \times K$ index matrix.
Elements of this matrix correspond to indices of points which should be used to estimate the signal values at the corresponding kernel elements.
They are calculated using the operation-specific procedure (i.e. Equations \ref{eq:signal_nn}-\ref{eq:signal_gauss} and \ref{eq:2} for convolution and pooling respectively).
Given the index matrix, we can collect signals from the incoming feature map and execute the corresponding operations.
The whole process is illustrated in Figure~\ref{fig:implementation}.

Importantly, the structure of the index matrix does not depend on the signal values, same as indices of spatial neighbors in regular images do not depend on the pixel values.
This allows us to precompute these matrices in advance purely based on the geometrical structure of the point cloud.

